Diffusion in the Dark: A Diffusion Model for Low-Light Text Recognition

Capturing images is a key part of automation for high-level tasks such as scene text recognition. Low-light conditions pose a challenge for high-level perception stacks, which are often optimized on well-lit, artifact-free images. Reconstruction methods for low-light images can produce well-lit counterparts, but typically at the cost of high-frequency details critical for downstream tasks. We propose Diffusion in the Dark (DiD), a diffusion model for low-light image reconstruction for text recognition. DiD provides qualitatively competitive reconstructions with that of state-of-the-art (SOTA), while preserving high-frequency details even in extremely noisy, dark conditions. We demonstrate that DiD, without any task-specific optimization, can outperform SOTA low-light methods in low-light text recognition on real images, bolstering the potential of diffusion models to solve ill-posed inverse problems.

==> main/tables/baselines.tex <==
\begin{tabular}{l|ccc}
\hline\noalign{\smallskip}
Method & PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$\\
\noalign{\smallskip}
\hline
\noalign{\smallskip}

Zero-DCE ~\cite{guo2020zero} &14.86 & 0.54 & 0.33 \\

LIME ~\cite{guo2016lime} & 16.76 & 0.56 & 0.35 \\

EnlightenGAN ~\cite{jiang2021enlightengan} & 17.48 & 0.65 & 0.32 \\

RetinexNet ~\cite{wei2018deep} & 16.77 & 0.56 & 0.47 \\

RUAS ~\cite{liu2021retinex} & 18.23 & 0.72 & 0.35 \\

DRBN ~\cite{yang2020fidelity} & 20.13 & 0.83 & 0.16 \\

KinD ~\cite{zhang2019kindling} & 20.87 & 0.80 & 0.17 \\

KinD++ ~\cite{zhang2021beyond}& 21.30 & 0.82 & 0.16 \\

LLFlow ~\cite{wang2022low} & \textbf{25.19} & \textbf{0.93} & \textbf{0.11} \\ 

\noalign{\smallskip}
\hline
\noalign{\smallskip}
StarDiffusion~\cite{yuan2022learning} & 20.77 & 0.80 & *\\

DDRM ~\cite{kawar2022denoising}& 16.41 & 0.65 & 0.21 \\ 

LDM ~\cite{rombach2022high} & 21.41	& 0.75 & 0.23 \\ 

DiD (Ours) & \underline{23.97} & \underline{0.84} & \underline{0.12}\\
\hline
\end{tabular}


% \begin{tabular}{l|c|ccc}
% \hline\noalign{\smallskip}
% Method  & Training Set & PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$\\
% \noalign{\smallskip}
% \hline
% \noalign{\smallskip}
% Zero-DCE (\hyperlink{cite.guo2020zero}{Guo et al. 2020}) & SICE~\cite{cai2018learning} &  14.86 & 0.54 & 0.33 \\

% LIME (\hyperlink{cite.guo2016lime}{Guo, Li, and Ling, 2016}) & N/A & 16.76 & 0.56 & 0.35 \\

% EnlightenGAN (\hyperlink{cite.jiang2021enlightengan}{Jiang et al. 2021}) & RAISE~\cite{dang2015raise}, SICE, LOL~\cite{wei2018deep}, HDR images~\cite{kalantari2017deep} & 17.48 & 0.65 & 0.32 \\

% RetinexNet (\hyperlink{cite.wei2018deep}{Wei et al. 2018}) & LOL & 16.77 & 0.56 & 0.47 \\

% RUAS (\hyperlink{cite.liu2021retinex}{Liu et al. 2021}) & LOL & 18.23 & 0.72 & 0.35 \\

% DRBN (\hyperlink{cite.yang2020fidelity}{Yang et al. 2020}) & LOL & 20.13 & \underline{0.83} & 0.16 \\

% KinD (\hyperlink{cite.zhang2019kindling}{Zhang et al. 2019}) & LOL & 20.87 & 0.80 & 0.17 \\

% KinD++ (\hyperlink{cite.zhang2021beyond}{Zhang et al. 2021}) & LOL & \underline{21.30} & 0.82 & 0.16 \\

% LLFlow (\hyperlink{cite.wang2022low}{Wang et al. 2022})& LOL & \textbf{25.19} & \textbf{0.93} & \textbf{0.11} \\ 

% (Ours) & LOL & 20.53 & 0.82 & \underline{0.12}\\
% \hline
% \end{tabular}


==> main/tables/ocr.tex <==
\begin{tabular}{l|cc|cc|cc|cc}
\hline\noalign{\smallskip}
\multirow{2}{*}{Method} & \multicolumn{2}{c}{IIIT5K~\cite{mishra2012scene}} & \multicolumn{2}{c}{ICDAR13~\cite{karatzas2013icdar}} & \multicolumn{2}{c}{SVT~\cite{wang2011end}} & \multicolumn{2}{c}{SVTP~\cite{phan2013recognizing}}\\
& \%Acc $\uparrow$ & 1-NED $\uparrow$ & \%Acc $\uparrow$ & 1-NED $\uparrow$ & \%Acc $\uparrow$ & 1-NED $\uparrow$ & \%Acc $\uparrow$ & 1-NED $\uparrow$\\

\noalign{\smallskip}
\hline
\noalign{\smallskip}
LLFlow ~\cite{wang2022low} &  \textbf{98.57} & \textbf{99.64} & 96.35 & 98.18 & 96.14 & 98.49 & 88.69 & 95.36\\
DiD (Ours) & 98.00 & 99.53 & \textbf{97.93} & \textbf{99.36} & \textbf{97.68} & \textbf{99.30} & \textbf{93.80} & \textbf{98.08}\\
\hline
\end{tabular}

